Results from an Einstein@Home search for continuous gravitational waves from G347.3 at low frequencies in LIGO O2 data

We present results of a search for periodic gravitational wave signals with frequency between 20 and 400 Hz, from the neutron star in the supernova remnant G347.3-0.5, using LIGO O2 public data. The search is deployed on the volunteer computing project Einstein@Home, with thousands of participants donating compute cycles to make this endevour possible. We find no significant signal candidate and set the most constraining upper limits to date on the amplitude of gravitational wave signals from the target, corresponding to deformations below $10^{-6}$ in a large part of the band. At the frequency of best strain sensitivity, near $166$ Hz, we set 90\%\ confidence upper limits on the gravitational wave intrinsic amplitude of $h_0^{90\%}\approx 7.0\times10^{-26}$. Over most of the frequency range our upper limits are a factor of 20 smaller than the indirect age-based upper limit.

==> paperBib.tex <==
\def\etal{{\it et al.}}

%%emission
\bibitem{Ushomirsky:2000ax} 
  G.~Ushomirsky, C.~Cutler and L.~Bildsten,
  ``Deformations of accreting neutron star crusts and gravitational wave emission,''
  Mon.\ Not.\ Roy.\ Astron.\ Soc.\  {\bf 319}, 902 (2000)
  doi:10.1046/j.1365-8711.2000.03938.x
  [astro-ph/0001136].
  
\bibitem{Andersson:1997rn} 
  N.~Andersson and K.~D.~Kokkotas,
  ``Towards gravitational wave asteroseismology,''
  Mon.\ Not.\ Roy.\ Astron.\ Soc.\  {\bf 299}, 1059 (1998)
  doi:10.1046/j.1365-8711.1998.01840.x
  [gr-qc/9711088].

\bibitem{Andersson:1998ze} 
  N.~Andersson, K.~D.~Kokkotas and B.~F.~Schutz,
  ``Gravitational radiation limit on the spin of young neutron stars,''
  Astrophys.\ J.\  {\bf 510}, 846 (1999)
  doi:10.1086/306625
  [astro-ph/9805225].
  
\bibitem{Owen:2010ng} 
  B.~J.~Owen,
  ``How to adapt broad-band gravitational-wave searches for r-modes,''
  Phys.\ Rev.\ D {\bf 82}, 104002 (2010)
  doi:10.1103/PhysRevD.82.104002
  [arXiv:1006.1994 [gr-qc]].

\bibitem{Watts:2008qw} 
  A.~Watts, B.~Krishnan, L.~Bildsten and B.~F.~Schutz,
  ``Detecting gravitational wave emission from the known accreting neutron stars,''
  Mon.\ Not.\ Roy.\ Astron.\ Soc.\  {\bf 389}, 839 (2008)
  doi:10.1111/j.1365-2966.2008.13594.x
  [arXiv:0803.4097 [astro-ph]].
  
\bibitem{Gualtieri:2010md} 
  L.~Gualtieri, R.~Ciolfi and V.~Ferrari,
  ``Structure, Deformations and Gravitational Wave Emission of Magnetars,''
  Class.\ Quant.\ Grav.\  {\bf 28}, 114014 (2011)
  doi:10.1088/0264-9381/28/11/114014
  [arXiv:1011.2778 [astro-ph.SR]].
 
\bibitem{Ciolfi:2013dta} 
  R.~Ciolfi and L.~Rezzolla,
  ``Twisted-torus configurations with large toroidal magnetic fields in relativistic stars,''
  Mon.\ Not.\ Roy.\ Astron.\ Soc.\  {\bf 435}, L43 (2013)
  doi:10.1093/mnrasl/slt092
  [arXiv:1306.2803 [astro-ph.SR]].

\bibitem{Glampedakis:2015fja} 
  K.~Glampedakis and P.~Lasky,
  %``Persistent crustÐcore spin lag in neutron stars,''
  Mon.\ Not.\ Roy.\ Astron.\ Soc.\  {\bf 450}, no. 2, 1638 (2015)
  doi:10.1093/mnras/stv638
  [arXiv:1501.05473 [astro-ph.SR]].

\bibitem{Cutler:2002nw} 
  C.~Cutler,
  %``Gravitational waves from neutron stars with large toroidal B fields,''
  Phys.\ Rev.\ D {\bf 66}, 084025 (2002)
  doi:10.1103/PhysRevD.66.084025
  [gr-qc/0206051].

\bibitem{vanEysden:2008pd} 
  C.~A.~van Eysden and A.~Melatos,
  %``Gravitational radiation from pulsar glitches,''
  Class.\ Quant.\ Grav.\  {\bf 25}, 225020 (2008)
  doi:10.1088/0264-9381/25/22/225020
  [arXiv:0809.4352 [gr-qc]].
  
\bibitem{Singh:2016ilt} 
  A.~Singh,
  %``Gravitational wave transient signal emission via Ekman pumping in neutron stars during post-glitch relaxation phase,''
  Phys.\ Rev.\ D {\bf 95}, no. 2, 024022 (2017)
  doi:10.1103/PhysRevD.95.024022
  [arXiv:1605.08420 [gr-qc]].
  
  
\bibitem{Haskell:2015jra} 
  B.~Haskell and A.~Melatos,
  ``Models of Pulsar Glitches,''
  Int.\ J.\ Mod.\ Phys.\ D {\bf 24}, no. 03, 1530008 (2015)
  doi:10.1142/S0218271815300086
  [arXiv:1502.07062 [astro-ph.SR]].


\bibitem{McDanielJohnsonOwen} Maximum elastic deformations of relativistic stars, N.K.~Johnson-McDaniel and B.J.~Owen, Phys.\ Rev.\ D {\bf 88} 044004 (2013).

\bibitem{Abbott:2018qee} 
  B.~P.~Abbott {\it et al.} [LIGO Scientific and Virgo Collaborations],
  ``Searches for Continuous Gravitational Waves from Fifteen Supernova Remnants and Fomalhaut b with Advanced LIGO,''
  arXiv:1812.11656 [astro-ph.HE].

\bibitem{S6EHCasA} 
  S.~J.~Zhu {\it et al.} 
``An Einstein@Home search for continuous gravitational waves from Cassiopeia A'',
  Phys.\ Rev.\ D {\bf 94}, 082008 (2016)

\bibitem{Aasi:2014ksa}
  J.~Aasi {\it et al.} [LIGO Scientific Collaboration],
  ``Searches for continuous gravitational waves from nine young supernova remnants'',
  Astrophys.\ J.\  {\bf 813} (2015) no.1,  39
  doi:10.1088/0004-637X/813/1/39
  [arXiv:1412.5942 [astro-ph.HE]].
  %%CITATION = doi:10.1088/0004-637X/813/1/39;%%
  %39 citations counted in INSPIRE as of 19 Feb 2019

\bibitem{Abadie:2010hv} 
  J.~Abadie {\it et al.} [LIGO Scientific Collaboration],
  ``First search for gravitational waves from the youngest known neutron star,''
  Astrophys.\ J.\  {\bf 722}, 1504 (2010)
  doi:10.1088/0004-637X/722/2/1504
  [arXiv:1006.2535 [gr-qc]].

\bibitem{Ming:2015jla} 
J.~Ming, B.~Krishnan, M.~A.~Papa, C.~Aulbert and H.~Fehrmann,
``Optimal directed searches for continuous gravitational waves,''
Phys.\ Rev.\ D {\bf 93}, 064011 (2016)
%Phys.\ Rev.\ D {\bf 93}, no. 6, 064011 (2016)
%doi:10.1103/PhysRevD.93.064011
%[arXiv:1510.03417 [gr-qc]].  

\bibitem{thankslosc}
M.~ Vallisneri {\it et al.} , "The LIGO Open Science Center",
Proceedings of the 10th LISA Symposium, 
arxiv:1410.4839, (2014).

\bibitem{O1data}
{\texttt{https://doi.org/10.7935/K57P8W9D}}, (2018).

\bibitem{Ming:2017anf}
  J.~Ming {\it et al.},
  ``Optimally setting up directed searches for continuous gravitational waves in Advanced LIGO O1 data,''
  Phys.\ Rev.\ D {\bf 97} (2018) no.2,  024051
  doi:10.1103/PhysRevD.97.024051
  [arXiv:1708.02173 [gr-qc]].
  %%CITATION = doi:10.1103/PhysRevD.97.024051;%%
  %4 citations counted in INSPIRE as of 18 Mar 2019


\bibitem{ATLAS}
\texttt{http://www.aei.mpg.de/24838/02} Computing and ATLAS

\bibitem{LIGO_detector} 
LIGO Scientific Collaboration,
``LIGO: The Laser Interferometer Gravitational-Wave Observatory"
 Rep. Prog. Phys. 72(2009) 076901



\bibitem{LIGO_O1} 
B.~Abbott \etal\ (LIGO Scientific Collaboration),
``GW150914: The Advanced LIGO Detectors in the Era of First Discoveries'',
 Phys.\ Rev.\ Lett.\ {\bf 116}, 131103 (2016).

%16 O1
\bibitem{TheLIGOScientific:2014jea} 
  J.~Aasi {\it et al.} (LIGO Scientific Collaboration),
  ``Advanced LIGO,''
  Class.\ Quant.\ Grav.\  {\bf 32}, 074001 (2015)
  doi:10.1088/0264-9381/32/7/074001
%  [arXiv:1411.4547 [gr-qc]].
  %%CITATION = doi:10.1088/0264-9381/32/7/074001;%%
  %207 citations counted in INSPIRE as of 01 Jun 2016

\bibitem{o1_data} https://doi.org/10.7935/CA75-FM95LIGO Open Science Center, \url{https://losc.ligo.org}.
%\bibitem{o2data} \url{doi.org/10.7935/CA75-FM95} LIGO Open Science Center, \url{https://losc.ligo.org}.

\bibitem{aligo} Advanced LIGO, J.~Aasi \etal\ (LIGO Scientific Collaboration), Class.\ Quantum Grav.\  {\bf 32} 7 (2015) .

\bibitem{SFTs}
B.~Allen and G.~Mendell, "SFT Data Format Version 2Specification", (2004), 
\texttt{https://dcc.ligo.org/LIGO-T040164/public}

\bibitem{Abbott:2017pqa}
  B.~P.~Abbott {\it et al.} [LIGO Scientific and Virgo Collaborations],
  ``First low-frequency Einstein@Home all-sky search for continuous gravitational waves in Advanced LIGO data,''
  Phys.\ Rev.\ D {\bf 96} (2017) no.12,  122004
  doi:10.1103/PhysRevD.96.122004
  [arXiv:1707.02669 [gr-qc]].
  %%CITATION = doi:10.1103/PhysRevD.96.122004;%%
  %15 citations counted in INSPIRE as of 19 Feb 2019


\bibitem{Jaranowski:1998qm}
  P.~Jaranowski, A.~Krolak and B.~F.~Schutz,
  ``Data analysis of gravitational - wave signals from spinning neutron stars. 1. The Signal and its detection,''
  Phys.\ Rev.\ D {\bf 58} (1998) 063001
  doi:10.1103/PhysRevD.58.063001
  [gr-qc/9804014].
  %%CITATION = doi:10.1103/PhysRevD.58.063001;%%
  %363 citations counted in INSPIRE as of 19 Feb 2019




\bibitem{PletschAllen}
H.~J.~Pletsch, B. Allen, 
``Exploiting Large-Scale Correlations to Detect Continuous Gravitational Waves''
Phys. Rev. Lett. {\bf 103}, 181102 (2009)

%17 O1
\bibitem{Pletsch:2008} 
  H.~J.~Pletsch,
  ``Parameter-space correlations of the optimal statistic for continuous gravitational-wave detection,''
  Phys.\ Rev.\ D {\bf 78}, 102005 (2008)
%  [arXiv:0807.1324 [gr-qc]].
  
 %18 O1
  \bibitem{Pletsch:2010} 
  H.~J.~Pletsch,
  ``Parameter-space metric of semicoherent searches for continuous gravitational waves,''
  Phys.\ Rev.\ D {\bf 82}, 042002 (2010)
%  [arXiv:1005.0395 [gr-qc]].

\bibitem{Cutler:2005hc}
  C.~Cutler and B.~F.~Schutz,
  ``The Generalized F-statistic: Multiple detectors and multiple GW pulsars,''
  Phys.\ Rev.\ D {\bf 72} (2005) 063006
  doi:10.1103/PhysRevD.72.063006
  [gr-qc/0504011].
  %%CITATION = doi:10.1103/PhysRevD.72.063006;%%
  %86 citations counted in INSPIRE as of 19 Feb 2019

%21 O1 (following counts are wrong)
\bibitem{Keitel:2013}
  D.~Keitel, R.~Prix, M.~A.~Papa, P.~Leaci and M.~Siddiqi,
  ``Search for continuous gravitational waves: Improving robustness versus instrumental artifacts,''
  Phys.\ Rev.\ D {\bf 89}, 064023 (2014)
%  Phys.\ Rev.\ D {\bf 89}, no. 6, 064023 (2014)
%  [arXiv:1311.5738 [gr-qc]].


%20 O1
\bibitem{Keitel:2016} 
  D.~Keitel,
  ``Robust semicoherent searches for continuous gravitational waves with noise and signal models including hours to days long transients'',
  Phys.\ Rev.\ D {\bf 93}, 084024 (2016)

\bibitem{Boinc1}
\texttt{http://boinc.berkeley.edu/}

\bibitem{Boinc2}
D.~P.~Anderson,
``BOINC: A System for Public-Resource Computing and Storage''
Proceedings of the Fifth IEEE/ACM International Workshop on Grid Computing (GRID04), pp. 4-10 (2004)

\bibitem{Boinc3}
D.~P.~Anderson, C.~Christensen, and B.~Allen,
``Designing a Runtime System for Volunteer Computing''
Proceedings of the 2006 ACM/IEEE conference on Supercomputing, pp.126-136 (2006)

\bibitem{Aasi:2015rar} 
  J.~Aasi {\it et al.} [LIGO Scientific and VIRGO Collaborations],
  ``First low frequency all-sky search for continuous gravitational wave signals,''
  Phys.\ Rev.\ D {\bf 93}, 042007 (2016)
%  Phys.\ Rev.\ D {\bf 93}, no. 4, 042007 (2016)
%  doi:10.1103/PhysRevD.93.042007

\bibitem{Dergachev:2019pgs}
  V.~Dergachev, M.~A.~Papa, B.~Steltner and H.~B.~Eggenstein,
  ``Loosely coherent search in LIGO O1 data for continuous gravitational waves from Terzan 5 and the galactic center,''
  arXiv:1903.02389 [gr-qc].

\bibitem{S6EHFU} 
 M.~A.~Papa {\it et al.} 
``Hierarchical follow-up of sub-threshold candidates of an all-sky Einstein@Home search for continuous gravitational waves on LIGO sixth science run data'', Phys.\ Rev.\ D {\bf 94}, 122006 (2016).


\bibitem{O2AllSkyLVC}
B.~P.~Abbott {\it et al.} [LIGO Scientific and Virgo Collaborations],
 All-sky search for continous gravitational waves from isolated neutron stars using Advanced LIGO O2 data,
 arXiv:1903:01901

\bibitem{Singh:2017kss}
  A.~Singh, M.~A.~Papa, H.~B.~Eggenstein and S.~Walsh,
  ``Adaptive clustering procedure for continuous gravitational wave searches,''
  Phys.\ Rev.\ D {\bf 96} (2017) no.8,  082003
  doi:10.1103/PhysRevD.96.082003
  [arXiv:1707.02676 [gr-qc]].


\bibitem{Zhu:2017ujz} 
  S.~J.~Zhu, M.~A.~Papa and S.~Walsh,
  ``New veto for continuous gravitational wave searches,''
  Phys.\ Rev.\ D {\bf 96}, no. 12, 124007 (2017)
  doi:10.1103/PhysRevD.96.124007
  [arXiv:1707.05268 [gr-qc]].
  %%CITATION = doi:10.1103/PhysRevD.96.124007;%%
  %3 citations counted in INSPIRE as of 12 Mar 2019
 
\bibitem{DMoff-sc}
 S.~J.~Zhu, D. Singh, and M.~A.~Papa, in preparation. 

\bibitem{AvneetThesis}
Avneet Singh, ``Improved post-processing in searches for continuous gravitational waves'', Chapter 5, Gottfried Wilhelm Leibniz Universitaet, PhD Diss., 2017, 140 S (DOI: https://doi.org/10.15488/3426)

\bibitem{GalacticCenterMethod} 
  B.~Behnke, M.~A.~Papa and R.~Prix,
 ``Postprocessing methods used in the search for continuous gravitational-wave signals from the Galactic Center,''
  Phys.\ Rev.\ D {\bf 91}, 064007 (2015)
%  Phys.\ Rev.\ D {\bf 91}, no. 6, 064007 (2015)
  doi:10.1103/PhysRevD.91.064007
%  [arXiv:1410.5997 [gr-qc]].


\bibitem{Dreissigacker:2018afk} 
  C.~Dreissigacker, R.~Prix and K.~Wette,
  ``Fast and Accurate Sensitivity Estimation for Continuous-Gravitational-Wave Searches",
  Phys.\ Rev.\ D {\bf 98}, no. 8, 084058 (2018)
%  doi:10.1103/PhysRevD.98.084058
%  [arXiv:1808.02459 [gr-qc]].
  %%CITATION = doi:10.1103/PhysRevD.98.084058;%%
  %4 citations counted in INSPIRE as of 01 Mar 2019


\bibitem{AEIULurl}
{\texttt{www.aei.mpg.de/continuouswaves/O1GY-DirectedSearches}}

\bibitem{Allen:2014yra} 
  G.~E.~Allen, K.~Chow, T.~DeLaney, M.~D.~Filipovic, J.~C.~Houck, T.~G.~Pannuti and M.~D.~Stage,
  ``On the Expansion Rate, Age, and Distance of the Supernova Remnant G266.2-1.2 (Vela Jr.),''
  Astrophys.\ J.\  {\bf 798}, no. 2, 82 (2015)
  doi:10.1088/0004-637X/798/2/82
  [arXiv:1410.7435 [astro-ph.HE]].
  %%CITATION = doi:10.1088/0004-637X/798/2/82;%%
  %21 citations counted in INSPIRE as of 19 Mar 2019

\bibitem{zimmermann:1979}
M.~ Zimmermann and E.~Szedenits, 
``Gravitational waves from rotating and precessing rigid bodies: Simple models and applications to pulsars",
Phys. Rev. D {\bf 20}, 351, (1979)


%%%%%%%%%%



